Federated Adversarial Learning: A Framework with Convergence Analysis

Federated learning (FL) is a trending training paradigm to utilize decentralized training data. FL allows clients to update model parameters locally for several epochs, then share them to a global model for aggregation. This training paradigm with multi-local step updating before aggregation exposes unique vulnerabilities to adversarial attacks. Adversarial training is a popular and effective method to improve the robustness of networks against adversaries. In this work, we formulate a general form of federated adversarial learning (FAL) that is adapted from adversarial learning in the centralized setting. On the client side of FL training, FAL has an inner loop to generate adversarial samples for adversarial training and an outer loop to update local model parameters. On the server side, FAL aggregates local model updates and broadcast the aggregated model. We design a global robust training loss and formulate FAL training as a min-max optimization problem. Unlike the convergence analysis in classical centralized training that relies on the gradient direction, it is significantly harder to analyze the convergence in FAL for three reasons: 1) the complexity of min-max optimization, 2) model not updating in the gradient direction due to the multi-local updates on the client-side before aggregation and 3) inter-client heterogeneity. We address these challenges by using appropriate gradient approximation and coupling techniques and present the convergence analysis in the over-parameterized regime. Our main result theoretically shows that the minimum loss under our algorithm can converge to $\epsilon$ small with chosen learning rate and communication rounds. It is noteworthy that our analysis is feasible for non-IID clients.

==> convergence.tex <==
\subsection{Convergence}
\label{sec:converge}




\Orestis{todo: 1. lemma+definition seem out of nowhere->set the stage, say what you will do. 2. missing definition of gradient and pseudonet gradient 3. $W^*$ undefined 4. $a_r~\{\pm 1/m^{1/3}\}$ 5. Initialization is $W^{ij}\sim N(0,1/m)$ 6.In my part I have written $\ind\{abc\}$ instead of $\ind_{abc}$}

\Orestis{missing notation: S(t), $\tilde{\ell}$, write guarantee for $min_t$ as in the other paper. Missing definition of pseudoloss}
\Yi{w.h.p. of initilization}
\begin{theorem}

\end{theorem}
\begin{proof}
For simplicity, in the proof we use the following shorthand notations to denote various distances.
\begin{itemize}[noitemsep,topsep=0pt]
    \item[] $D_{\text{max}}:= \max_{ t \in [T] }\|W^{(t)} - W^{(0)}\|_{2,\infty}$
    \item[] $D_{W^{*}}:= \|W^{*} - W^{(0)}\|_{2,\infty}$
\end{itemize}
By condition, we know $D_{W^*}=O\left(\frac{R}{m^{2/3}}\right)$.
Even though in Algorithm~\ref{alg:adv-train} the parameters $W$ are updated using the gradients of the \emph{real net}, in this proof we consider the pseudo-net as the object being optimized. Thus we need to relate the real net gradients to the pseudo-net gradients. For ease of presentation, we define the following convenient notations for the two notions of gradients:
\begin{itemize}[noitemsep,topsep=0pt]
    \item[] real net gradient $\nabla^{(t)}:=\nabla_W\mathcal{L}(f(W^{(t)}), S^{(t)})$ 
    \item[] pseudo-net gradient $\hat{\nabla}^{(t)}:=\nabla_W\mathcal{L}(g(W^{(t)}), S^{(t)})$
\end{itemize}
In fact, by Lemma~\ref{lemma:coupling}, we know that they are coupled w.h.p. as long as $W^{(t)}$ stays close to initialization (i.e., $D_{\max}\leq m^{-7/12}$).
\begin{align*}
      \| \hat{\nabla}^{(t)} - \nabla^{(t)} \|_{2,1} \leq O\left(Lnm^{7/12}\right) \| W^{(t)} - W^{(0)}\|_{2,\infty}
\end{align*}
\begin{remark}
We assume for now $D_{\max}\leq m^{-7/12}$ is true and in the end we will set proper values for $T, \eta$ and $m$ to make sure this is indeed the case.
\end{remark}
Furthermore we note there is an upper bound on the gradient size:
\begin{align}\label{ineq:gradient-size}
    \|\nabla^{(t)}_r\|_2 &\leq L |a_r| \left(\frac{1}{n}\sum_{i=1}^n \sigma'\left(\inner{W^{(t)}_r}{x_i}+b_r^{(0)}\right)\|x_i\|_2\right) \notag\\
    &\leq \frac{L}{m^{1/3}}
\end{align}

Due to the linearity of $g$ with respect to $W$, the loss $\mathcal{L}(g(W), S)$ is in fact convex in $W$. We proceed to exploit the convexity and swap in the real net gradient:
\begin{align*}
    & ~ \mathcal{L}(g(W^{(t)}), S^{(t)}) - \mathcal{L}(g(W^*), S^{(t)}) \\
    \leq & ~\inner{\nabla^{(t)}}{W^{(t)} - W^*} + \inner{\hat{\nabla}^{(t)} - \nabla^{(t)}}{W^{(t)} - W^*} \\
    \leq & ~ \underbrace{\inner{\nabla^{(t)}}{W^{(t)} - W^*}}_{:=\text{\textalpha}^{(t)}}  \\
    &~~~~~~~~~~~~~~~~~~~~+ \underbrace{\|\hat{\nabla}^{(t)} - \nabla^{(t)}\|_{2,1}\|W^{(t)} - W^* \|_{2,\infty}}_{:=\text{\textbeta}^{(t)}}
\end{align*}
Then we deal with \textalpha~and~\textbeta~terms separately. As for the former, we use the standard online gradient descent proof technique:
\begin{align*}
\text{\textalpha}^{(t)} &\leq \frac{\eta}{2} \| \nabla^{(t)} \|_F^2 + \frac{\| W^{(t)} - W^* \|_F^2 - \| W^{(t+1)} - W^* \|_F^2}{2\eta} 
\end{align*}
We then sum over time indices $t$ and take care of the telescopic terms:
\begin{align*}
\sum_{t=1}^T \text{\textalpha}^{(t)} &\leq \frac{\eta}{2}\left(\sum_{t=1}^T\|\nabla^{(t)}\|_F^2\right) + \frac{\| W^* -  W^{(0)}\|_F^2}{2\eta} \\
&\leq \frac{\eta L^2 m^{1/3}}{2}T + \frac{m D_{W^*}^2}{2\eta}
\end{align*}
where we used the fact $\|W^* -  W^{(0)}\|_F^2\leq m\cdot \|W^* -  W^{(0)}\|_{2,\infty}=m D_{W^*}^2$ 
as well as $\|\nabla^{(t)}\|_F^2\leq \sum_{r=1}^m \|\nabla_r^{(t)}\|_2^2\leq L^2m^{1/3}$.

For the $\text{\textbeta}^{(t)}$'s, we first invoke Lemma~\ref{lemma:coupling} and then apply a simple triangle inequality:
\begin{align*}
\text{\textbeta}^{(t)} &\leq O\left(Lnm^{7/12}\right)\| W^{(t)} - W^* \|_{2,\infty}\\
&\leq O\left(Lnm^{7/12}\right) \left(D_{\text{max}} + D_{W^{*}}\right)
\end{align*}

Furthermore we can bound the size of $D_{\text{max}}$ using the bound on gradients, i.e. $\|\nabla^{(t)}_r\|_2\leq Lm^{-1/3}$ using Inequality~\ref{ineq:gradient-size}.
\begin{align*}
    D_{\text{max}} &= \max_{ t \in [T]}\|W^{(0)} - W^{(t)}\|_{2,\infty} \\
    &\leq \sum_{t=1}^T \eta \max_{r\in[m]}\|\nabla^{(t)}_r\|_2 \leq \frac{\eta L T}{m^{1/3}}
\end{align*}

Putting it together with the condition $D_{W*}=O\left(\frac{R}{m^{2/3}}\right)$ that we already have, we obtain the following:
\begin{align*}
    & ~ \sum_{t=1}^T  \mathcal{L}(g(W^{(t)}), S^{(t)}) - \sum_{t=1}^T \mathcal{L}(g(W^*), S^{(t)})\\ 
    \leq & \sum_{t=1}^T \text{\textalpha}^{(t)} + \sum_{t=1}^T \text{\textbeta}^{(t)} \\
    \leq & O\left(\eta L^2 T n m^{1/4} + \frac{\eta R L T n}{m^{1/12}}  +  m^{1/3} \eta L^2 T +  \frac{R^2}{m^{1/3} \eta}\right)
\end{align*}

Finally we arrive at the desired statement
\begin{align*}
   \frac{1}{T} \sum_{t=1}^T \mathcal{L}(g(W^{(t)}), S^{(t)}) - \frac{1}{T} \sum_{t=1}^T \mathcal{L}(g(W^*), S^{(t)}) &\leq \varepsilon
\end{align*}
if we set the hyper-parameters $T, m, \eta$ to be the following:
\begin{itemize}
    \item[] $T=\Theta( \epsilon^{-2} L^2R^2 )$,
    \item[] $m=\Omega\left(\max\left\{ \left(\frac{n}{\epsilon}\right)^{12}, \left(\frac{Rn}{L\epsilon}\right)^{12/5}, \left(\frac{R^2L}{\epsilon}\right)^{12} \right\} \right)$,
    \item[] $\eta=\frac{R}{m^{1/3} L \sqrt{T}}=\Theta(m^{-1/3} L^{-2} \epsilon )$  
\end{itemize}
Note the the requirement on $m$ is to satisfy $\eta L^2 T n m^{1/4} + \frac{\eta R L T n}{m^{1/12}} \leq O(\epsilon)$ and $D_{\max}\leq m^{-7/12}$.

\end{proof}

==> optional.tex <==
\section*{Ethics Statement}
Ensuring the security and robustness of the deployed algorithms is of paramount importance in AI algorithms nowadays. Recently, machine learning training has revealed its vulnerability to adversarial attacks and tendency to generate wrong predictions. The tread cannot be underestimated in FL, where the heterogeneity among clients and requirement for efficient communication brings in challenges in stable gradient updates. In this regard, our work theoretically shows the feasibility of FAL. As a theoretical work, we do not involve any human subjects or datasets. Our work has the potential positive impact on the machine learning community. 

\section*{Reproducibility Statement}
We provide the proof details in the appendix to ensure reproducibility.

==> social.tex <==
\section{Societal Impact}
\label{sec:impact}
Ensuring the security and robustness of the deployed algorithms is of paramount importance in AI algorithms nowadays. Recently, machine learning training reveals its vulnerability to adversarial attack and tendency to generate wrong predictions. The tread even cannot be underestimated in FL, where the heterogeneity among clients and requirement for efficient communication bring in challenges in stable gradient updates. 
 
A small mistake of the AI system for the above applications is fatal. Adversarial training has been used in classical training to improve model robustness. Thus, this motivates us to investigate the feasibility of adversarial training in FL from the aspect of theoretical convergence analysis. Our results show the plausible convergence properties with certain assumptions. This work will provide insights into applying adversarial training in FL and developing new algorithms. However, it is worth noting that the real application conditions can be way more complex than those in our theoretical analysis; thus, we did not aim to provide the practical convergence guarantee in the actual deployment. 




